On Rich Clubs of Path-Based Centralities in Networks

Many scale-free networks exhibit a rich club structure, where high degree vertices form tightly interconnected subgraphs. In this paper, we explore the emergence of rich clubs in the context of shortest path based centrality metrics. We term these subgraphs of connected high closeness or high betweeness vertices as rich centrality clubs (RCC). Our experiments on real world and synthetic networks highlight the inter-relations between RCCs, expander graphs, and the core-periphery structure of the network. We show empirically and theoretically that RCCs exist, if the core-periphery structure of the network is such that each shell is an expander graph, and their density decreases from inner to outer shells. The main contributions of our paper are: (i) we demonstrate that the formation of RCC is related to the core-periphery structure and particularly the expander like properties of each shell, (ii) we show that the RCC property can be used to find effective seed nodes for spreading information and for improving the resilience of the network under perturbation and, finally, (iii) we present a modification algorithm that can insert RCC within networks, while not affecting their other structural properties. Taken together, these contributions present one of the first comprehensive studies of the properties and applications of rich clubs for path based centralities.

==> experiments.tex <==
%\subsection{Centrality of the inner cores}
%\label{sec:super}
% We have observed from the experiments that in high expansion networks, a majority of the shortest paths in the network pass through the vertices in the inner cores. Let us consider the paths between two vertices in the context of their community assignments. Note that if two vertices are in the same community then, the shortest path between them is also likely to be within the community. Since the vertices in the inner cores of high expansion networks belong to multiple communities, it follows their centrality is achieved by connecting vertices across communities. Therefore {\em our hypothesis is that in  the high expansion networks most of the paths between communities pass through the inner cores.}

% \noindent{\bf Empirical corroboration}: To demonstrate that the paths between communities mostly pass through the innermost cores, we divide the vertices in the network into  two sets of nodes, based on whether they are part of the innermost core or not. We partition the nodes outside the innermost core into clusters using the Louvian algorithm~\cite{blondel2008fast}. Vertices in each cluster are combined into a single supervertex. The set of nodes of  the innermost core are also combined into a supervertex. Two supervertices are connected if there is at least one edge between the nodes comprising them. We compute the betweeness and closeness centrality of this reduced network.

% %Between each collapsed node we form an edge if atleast one pair of nodes are connected between them. Hence these nodes are connected by links weighted by number of edges connecting them. 

% %Without loss of generality, we consider inter community information propagation is dependent on the inner shell nodes if they are close to all the clusters as well as they lie on the shortest paths between two nodes in separate communities. We estimate the non overlaping communities in the network using \cite{blondel2008fast} louvian method. We partition the nodes in the network($V$) into inner most shell nodes ($K$) and remaining nodes ($C$) of the network. This set $K$ an also be formed from multiple inner most shell nodes of the network. Each of the communities of the network ($c_1,c_2,...c_k$)is represented as a meta vertex. One set of edges connect two meta vertices which represent communities  and they comprise inter community edges which belong to nodes pertaining to the set $C$. A second type of  meta vertex is formed from nodes belong to the set $K$, and any edge joining vertex in $K$ to a community $c_i$ is represented as a meta edge. We finally obtain a meta network comprising of nodes equal to the number of communities and single she;; meta vertiex. This shell meta vertex may comprise a single shell or multiple shells. 

% Our results show that for high expansion networks, the supervertex representing the innermost core  has the largest centrality value with respect to both betweenness and closeness centrality for most of the high expansion networks. In contrast, in the other group of networks, this supervertex has much lower centrality. We provide two sets of results to support this statement.

% First, in Figure~\ref{fig:superv}, we present a visualization of the reduced network for two benchmark networks. Each node is labeled as $c_x$ for communities and $k$ for the innermost core. The supervertex with the largest average centrality (i.e., average of the closeness and the betweenness centralities) is annotated by a separate color and size.   % In case the meta vertex with only the inner most shell is not the top central node, including the nodes from the second inner most shel immediately ranks it as top central node in majority of our high expansion networks. This shows that seed nodes based on inner most shells are most efficient spreaders in terms of inter community edges i.e messages initiated at inner most shell nodes, quickly transmits the message via inter community edges to several clusters which result in fast dissemination. In case of the low expansion class of networks, meta vertex with respect to the inner most shell donot assume the highest rank with respect to the inner most shell for most networks and this is true even when collapsing subsequent shells. 

% Next, for each reduced network, we compute the centrality (betweenness and closeness) of all the supervertices. We rank each supervertex based on its centrality score. For each reduced network, if the supervertex corresponding to the innermost core is within the top 10 ranked supervertices, we report its reciprocal rank (1/rank) in Table~\ref{tab:mrr}; otherwise, if it is not within the top ten, we report zero. We see a striking difference between the high expansion networks (colored \textcolor{blue}{blue}) and the others (colored \textcolor{brown}{brown}). For the high expansion networks, the reciprocal rank of the supevertex corresponding to the innermost core is almost always one indicating that this supervertex is indeed the most central. {\em These results support our hypothesis that for high expansion networks most of the paths between communities, pass through the inner cores.}
%its shells are expander-like with the  expansion property gradually decreasing from inner to outer shells.} 


\begin{table}\small
\begin{tabular}{ |c|c|c| } 
 \hline
 Network & Closeness & Betweenness  \\ 
 \hline
 \textcolor{blue}{AS} & 1 & 0.5  \\ 
 \hline
 \textcolor{blue}{Caida} & 1 & 1  \\ 
 \hline
 \textcolor{blue}{Bible} & 1 & 1 \\ 
  \hline
 \textcolor{blue}{Software} & 1 & 1 \\ 
 \hline
 \hline
 \textcolor{brown}{Protein} & 0 & 0 \\ 
 \hline
 \textcolor{brown}{Hepth} & 0.5 & 0.33 \\ 
 \hline
 \textcolor{brown}{Power} & 0 & 0 \\ 
 \hline
 \textcolor{brown}{Facebook} & 0.5 & 0.5 \\ 
 \hline
 \hline
 \textcolor{blue}{N1} & 1 & 1 \\ 
 \hline
 \textcolor{blue}{N2} & 1 & 1 \\ 
 \hline
 \textcolor{blue}{N3} & 1 & 1 \\ 
 \hline
 \textcolor{blue}{N4} & 1 & 1 \\ 
 \hline
 \textcolor{blue}{N5} & 1 & 1 \\ 
 \hline
 \textcolor{blue}{N6} & 1 & 1 \\ 
 \hline
 \textcolor{blue}{N7} & 0.5 & 1 \\ 
 \hline
 \textcolor{blue}{N8} & 1 & 0.5 \\ 
 \hline
 \hline
 \textcolor{brown}{N9}  & 0 & 0 \\ 
 \hline
 \textcolor{brown}{N10} & 0 & 0 \\ 
 %\hline
% \textcolor{brown}{N11} & 0.5 & 0.33 \\
 \hline
%\textcolor{brown}{N11} & 0.33 & 0.33 \\ 
% \hline
 \textcolor{brown}{N12} & 0.33 & 0.5 \\ 
 \hline
 \textcolor{brown}{N13} & 0.5 & 0.5 \\ 
 \hline
 \textcolor{brown}{N14} & 0 & 0 \\ 
 \hline
 \textcolor{brown}{N15} & 0 & 0 \\ 
 \hline
\end{tabular}
\caption {\label{tab:mrr} Reciprocal rank of the supervertex corresponding to the innermost core of the network. The ranking in done both based on closeness (second column) as well as betweenness (third column) centrality.}
\end{table}


\begin{figure}[t!]
    \centering
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[height=1.5in]%{Figs/super_cai.pdf}
        {caida_su.png}
        \caption{Caida}
    \end{subfigure}%
    ~
    \begin{subfigure}[t]{0.25\textwidth}
        \centering
        \includegraphics[height=1.5in]%{Figs/super_pow.pdf}
        {pow_su.png}
        \caption{Power}
    \end{subfigure}%  
    \caption{\label{fig:superv}Derived network formed by two category of supervertices, i.e, communities (denoted by $c_1$, $c_2$, $\dots$) and the innermost core (denoted by $k$). Two supervertices are connected if the corresponding nodes from which they are formed are connected by at least an edge. Highest average central supervertex (average of the closeness and the betweenness centrality values) is annotated by a larger size and a different color.}
  \end{figure}

\input{Expansion}



 




